Deciding What to Learn: A Rate-Distortion Approach

Agents that learn to select optimal actions represent a prominent focus of the sequential decision-making literature. In the face of a complex environment or constraints on time and resources, however, aiming to synthesize such an optimal policy can become infeasible. These scenarios give rise to an important trade-off between the information an agent must acquire to learn and the sub-optimality of the resulting policy. While an agent designer has a preference for how this trade-off is resolved, existing approaches further require that the designer translate these preferences into a fixed learning target for the agent. In this work, leveraging rate-distortion theory, we automate this process such that the designer need only express their preferences via a single hyperparameter and the agent is endowed with the ability to compute its own learning targets that best achieve the desired trade-off. We establish a general bound on expected discounted regret for an agent that decides what to learn in this manner along with computational experiments that illustrate the expressiveness of designer preferences and even show improvements over Thompson sampling in identifying an optimal policy.

==> Blahut-Arimoto Satisficing Thompson Sampling/algorithms/blasts_alg.tex <==
\begin{algorithm}[tbh]
   \caption{Blahut-Arimoto Satisficing Thompson Sampling (BLASTS)}
   \label{alg:blasts}
\begin{algorithmic}
   \STATE {\bfseries Input:} Lagrange multiplier $\beta \in \bR_{\geq 0}$, Blahut-Arimoto iterations $K \in \bN$, Posterior samples $Z \in \bN$
   \STATE $H_0 = \{\}$
   \FOR{$t=0$ {\bfseries to} $T-1$}
   \STATE $e_1,\ldots,e_Z \sim \bP(\environment \in \cdot | H_t)$ \COMMENT{Finite sample from current belief over $\environment$}
   \STATE $d(a,e|H_t) = \E[(\overline{r}(A_\star) - \overline{r}(a))^2 | \environment = e, H_t])$ \COMMENT{Distortion function for target action $\tilde{A}_t$}
   \STATE $\tilde{p}_0(a| e_z) = \frac{1}{|\mc{A}|}, \forall a \in \mc{A}, z \in [Z]$
   \FOR{$k=0$ {\bfseries to} $K-1$}
   \STATE $\tilde{q}_k(a) = \E_t[\tilde{p}_k(a|\environment)], \forall a \in \actions$ \COMMENT{Run the Blahut-Arimoto algorithm}
   \STATE $\tilde{p}_{k+1}(a |e_z) = \frac{\tilde{q}_k(a) \exp(-\beta d(a,e_z \mid H_t))}{\sum_{a' \in \actions} \tilde{q}_k(a') \exp(-\beta d(a,e_z \mid H_t))}, \forall a \in \actions, z \in [Z]$ 
   \ENDFOR
   \STATE $\hat{z} \sim \text{Uniform}(Z)$ \COMMENT{Select posterior sample uniformly at random}
   \STATE $A_t \sim \tilde{p}_K(a|e_{\hat{z}})$\COMMENT{Probability matching}
   \STATE $H_{t+1} = H_t \cup \{(A_t,O_{t+1})\}$
   \STATE $R_{t+1} = r(A_t, O_{t+1})$
   \ENDFOR
\end{algorithmic}
\end{algorithm}

==> Blahut-Arimoto Satisficing Thompson Sampling/algorithms/blasts_alg_no_comments.tex <==
\begin{algorithm}[tbh]
   \caption{Blahut-Arimoto Satisficing Thompson Sampling (BLASTS)}
\begin{algorithmic}
   \STATE {\bfseries Input:} Lagrange multiplier $\beta \in \bR_{\geq 0}$, Blahut-Arimoto iterations $K \in \bN$, Posterior samples $Z \in \bN$
   \STATE $H_0 = \{\}$
   \FOR{$t=0$ {\bfseries to} $T-1$}
   \STATE $e_1,\ldots,e_Z \sim \bP(\environment \in \cdot | H_t)$
   \STATE $d(a,e|H_t) = \E[(\overline{r}(A_\star) - \overline{r}(a))^2 | \environment = e, H_t])$
   \STATE $\tilde{p}_0(a| e_z) = \frac{1}{|\mc{A}|}, \forall a \in \mc{A}, z \in [Z]$
   \FOR{$k=0$ {\bfseries to} $K-1$}
   \STATE $\tilde{q}_k(a) = \E_t[\tilde{p}_k(a|\environment)], \forall a \in \actions$
   \STATE $\tilde{p}_{k+1}(a |e_z) \propto \tilde{q}_k(a) \exp\left(-\beta d(a,e_z \mid H_t)\right), \forall a \in \actions, \forall z \in Z$ 
   \ENDFOR
   \STATE $\hat{z} \sim \text{Uniform}(Z)$
   \STATE $A_t \sim \tilde{p}_K(a|e_{\hat{z}})$
   \STATE $H_{t+1} = H_t \cup \{(A_t,O_{t+1})\}$
   \STATE $R_{t+1} = r(A_t, O_{t+1})$
   \ENDFOR
\end{algorithmic}
 \label{alg:blasts}
\end{algorithm}

==> Blahut-Arimoto Satisficing Thompson Sampling/commands.tex <==
% Dynamically sized mid bar.
\newcommand{\bigmid}{\mathrel{\Big|}}

% ---- Colors and Notes ----
\definecolor{dblue}{RGB}{98, 140, 190}
\definecolor{dlblue}{RGB}{216, 235, 255}
\definecolor{dgreen}{RGB}{124, 155, 127}
\definecolor{dpink}{RGB}{207, 166, 208}
\definecolor{dyellow}{RGB}{255, 248, 199}
\definecolor{dgray}{RGB}{46, 49, 49}

% URL
\newcommand{\durl}[1]{\textcolor{dblue}{\underline{\url{#1}}}}

% Circled Numbers
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=0.7pt] (char) {\footnotesize{#1}};}}
% From: http://tex.stackexchange.com/questions/7032/good-way-to-make-textcircled-numbers

% Under set numbered subset of equation
\newcommand{\numeq}[3]{\underset{\textcolor{#2}{\circled{#1}}}{\textcolor{#2}{#3}}}

% ---- Abbreviations -----
\newcommand{\tc}[2]{\textcolor{#1}{#2}}
\newcommand{\ubr}[1]{\underbrace{#1}}
\newcommand{\uset}[2]{\underset{#1}{#2}}
\newcommand{\eps}{\varepsilon}

% Typical limit:
\newcommand{\nlim}{\underset{n \rightarrow \infty}{\lim}}
\newcommand{\nsum}{\sum_{i = 1}^n}
\newcommand{\nprod}{\prod_{i = 1}^n}

% Add an hrule with some space
\newcommand{\spacerule}{\begin{center}\hdashrule{2cm}{1pt}{1pt}\end{center}}

% Mathcal and Mathbb
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mf}[1]{\mathfrak{#1}}
\newcommand{\indic}{\mathbbm{1}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bV}{\mathbb{V}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\bI}{\mathbb{I}}
\newcommand{\bH}{\mathbb{H}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bF}{\mathbb{F}}
\newcommand{\bZ}{\mathbb{Z}}
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\rank}{\text{rank}}
\newcommand{\kl}[2]{D_{\mathrm{KL}}(#1 || #2)}
\newcommand{\expect}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\variance}[1]{\mathbb{V}\left[#1\right]}
\newcommand{\covar}[1]{Cov\left[#1\right]}

\DeclareMathOperator*{\esssup}{ess\,sup}

\newcommand{\ra}{\rightarrow}
\newcommand{\la}{\leftarrow}

% argmin, argmax.
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

% ---- Figures, Boxes, Theorems, Etc. ----

% Basic Image
\newcommand{\img}[2]{
\begin{center}
\includegraphics[scale=#2]{#1}
\end{center}}

% Put a fancy box around things.
\newcommand{\dbox}[1]{
\begin{mdframed}[roundcorner=4pt, backgroundcolor=gray!5]
\vspace{1mm}
{#1}
\end{mdframed}
}

%  --- PROOFS ---

% Inner environment for Proofs
\newmdenv[
  topline=false,
  bottomline=false,
  rightline = false,
  leftmargin=10pt,
  rightmargin=0pt,
  innertopmargin=0pt,
  innerbottommargin=0pt
]{innerproof}

% Proof Command
%\newenvironment{dproof}{\begin{proof} \text{\vspace{2mm}} \begin{innerproof}}{\end{innerproof}\end{proof}\vspace{4mm}}
\newenvironment{dproof}[1][Proof]{\begin{proof}[#1] \text{\vspace{2mm}} \begin{innerproof}}{\end{innerproof}\end{proof}\vspace{4mm}}


% Dave Definition
\newcounter{DaveDefCounter}
\setcounter{DaveDefCounter}{1}

\newcommand{\ddef}[2]
{
\begin{mdframed}[roundcorner=1pt, backgroundcolor=white]
\vspace{1mm}
{\bf Definition \theDaveDefCounter} (#1): {\it #2}
\stepcounter{DaveDefCounter}
\end{mdframed}
}

% Block Quote
\newenvironment{dblockquote}[2]{
\begin{blockquote}
#2
\vspace{-2mm}\hspace{10mm}{#1} \\
\end{blockquote}}

% Algorithm
\newenvironment{dalg}[1]
{\begin{algorithm}\caption{#1}\begin{algorithmic}}
{\end{algorithmic}\end{algorithm}}

% Dave Table
\newenvironment{dtable}[1]
{\begin{figure}[h]
\centering
\begin{tabular}{#1}\toprule}
{\bottomrule
\end{tabular}
\end{figure}}

% For numbering the last of an align*
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}



\newtheorem{assumption}{Assumption}
\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}{Corollary}
\newtheorem{claim}{Claim}
\newtheorem{example}{Example}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{theorem}{Theorem}
\newtheorem{fact}{Fact}
\newtheorem{question}{Question}

==> Blahut-Arimoto Satisficing Thompson Sampling/proofs/corollary2.tex <==
\begin{dproof}
\begin{align*}
    \E_\tau\left[\sum_{t=\tau}^\infty \mathbb{I}_t(\tilde{A}_t; (A_t, O_{t+1}))\right] &\leq \E_\tau\left[\sum_{t=\tau}^\infty \mc{L}_\beta(\tilde{A}_t|H_t) - \bE_t\left[\mc{L}_\beta(\tilde{A}_{t+1}|H_{t+1})\right]\right] \\
    &= \sum_{t=\tau}^\infty \bE_\tau\left[\mc{L}_\beta(\tilde{A}_t|H_t) \right] - \bE_\tau\left[\bE_t\left[\mc{L}_\beta(\tilde{A}_{t+1}|H_{t+1})\right]\right] \\
    &= \bE_\tau\left[\mc{L}_\beta(\tilde{A}_\tau|H_\tau)\right] + \sum_{t=\tau+1}^\infty \bE_\tau\left[\mc{L}_\beta(\tilde{A}_t|H_t) \right] - \sum_{t=\tau}^\infty \bE_\tau\left[\mc{L}_\beta(\tilde{A}_{t+1}|H_{t+1}) \right] \\
    &= \mc{L}_\beta(\tilde{A}_\tau|H_\tau) + \sum_{t=\tau+1}^\infty \bE_\tau\left[\mc{L}_\beta(\tilde{A}_t|H_t) \right] - \sum_{t=\tau+1}^\infty \bE_\tau\left[\mc{L}_\beta(\tilde{A}_{t}|H_{t}) \right] \\
    &= \mc{L}_\beta(\tilde{A}_\tau|H_\tau) \leq \mc{L}_\beta(\tilde{A}|H_\tau)
\end{align*}

where the steps follow as Lemma \ref{le:adapt_targets}, linearity of expectation, the tower property, and the fact that $\tilde{A}_\tau$ is the minimizer of $\mc{L}_\beta(\cdot|H_\tau)$, by definition.
\end{dproof}

==> Blahut-Arimoto Satisficing Thompson Sampling/proofs/corollary3.tex <==
\begin{dproof}
\begin{align*}
    \E_\tau\left[\sum_{t=\tau}^{T + \tau} \mathbb{I}_t(\tilde{A}_t; (A_t, O_{t+1}))\right] &\leq \E_\tau\left[\sum_{t=\tau}^{T + \tau} \mc{L}_\beta(\tilde{A}_t|H_t) - \bE_t\left[\mc{L}_\beta(\tilde{A}_{t+1}|H_{t+1})\right]\right] \\
    &= \sum_{t=\tau}^{T + \tau} \bE_\tau\left[\mc{L}_\beta(\tilde{A}_t|H_t) \right] - \bE_\tau\left[\bE_t\left[\mc{L}_\beta(\tilde{A}_{t+1}|H_{t+1})\right]\right] \\
    &= \bE_\tau\left[\mc{L}_\beta(\tilde{A}_\tau|H_\tau)\right] + \sum_{t=\tau+1}^{T + \tau} \bE_\tau\left[\mc{L}_\beta(\tilde{A}_t|H_t) \right] - \sum_{t=\tau}^{T + \tau} \bE_\tau\left[\mc{L}_\beta(\tilde{A}_{t+1}|H_{t+1}) \right] \\
    &= \mc{L}_\beta(\tilde{A}_\tau|H_\tau) + \sum_{t=\tau+1}^{T + \tau} \bE_\tau\left[\mc{L}_\beta(\tilde{A}_t|H_t) \right] - \sum_{t=\tau+1}^{T + \tau + 1} \bE_\tau\left[\mc{L}_\beta(\tilde{A}_{t}|H_{t}) \right] \\
    &= \mc{L}_\beta(\tilde{A}_\tau|H_\tau) - \bE_\tau\left[\mc{L}_\beta(\tilde{A}_{T + \tau +1}|H_{T + \tau +1}) \right] \\
    &\leq \mc{L}_\beta(\tilde{A}_\tau|H_\tau) \leq \mc{L}_\beta(\tilde{A}|H_\tau)
\end{align*}

where the steps follow as Lemma \ref{le:adapt_targets}, linearity of expectation, the tower property, the non-negativity of $\mc{L}_\beta(\tilde{A}_{t}|H_{t}) \geq 0$, and the fact that $\tilde{A}_\tau$ is the minimizer of $\mc{L}_\beta(\cdot|H_\tau)$, by definition.
\end{dproof}

==> Blahut-Arimoto Satisficing Thompson Sampling/proofs/lemma1.tex <==
\begin{dproof}
Recall that $H_{t+1} = (H_t, A_t, O_{t+1})$.  By definition of a target action, we have that $\forall t, H_t \perp \tilde{A} | \environment$, which implies $\bI_t((A_t,O_{t+1});\tilde{A}|\environment) = 0$. Thus, $$\bI_t(\environment; \tilde{A}) = \bI_t(\environment; \tilde{A}) + \bI_t((A_t,O_{t+1});\tilde{A}| \environment) = \mathbb{I}_t(\environment, (A_t, O_{t+1}); \tilde{A})$$ by the chain rule of mutual information. Applying the chain rule once again, we have,
$$\mathbb{I}_t(\environment; \tilde{A}) = \mathbb{I}_t(\environment, (A_t, O_{t+1}); \tilde{A}) = \mathbb{I}_t(\environment; \tilde{A} |A_t, O_{t+1}) + \mathbb{I}_t(\tilde{A}; (A_t, O_{t+1})).$$
It follows that
\begin{align*}
\E_t[\mathcal{L}_\beta(\tilde{A} | H_{t+1})] =& 
\E[\mathcal{L}_\beta(\tilde{A} | H_{t+1}) | H_t] \\
=& \E\left[\mathbb{I}_t(\environment; \tilde{A} |A_t, O_{t+1}) +  \beta \E\left[(\overline{r}(A_\star) - \overline{r}(\tilde{A}))^2 | H_t, A_t, O_{t+1} \right] \Big| H_t\right] \\
=& \E_t\left[\mathbb{I}_t(\environment; \tilde{A} | A_t, O_{t+1}) \right] +  \beta \E_t\left[(\overline{r}(A_\star) - \overline{r}(\tilde{A}))^2 \right] \\
=& \E_t\left[\mathbb{I}_t(\environment; \tilde{A}) - \mathbb{I}_t(\tilde{A};(A_t, O_{t+1})) \right]  +  \beta \E_t\left[(\overline{r}(A_\star) - \overline{r}(\tilde{A}))^2 \right] \\
=& \mathbb{I}_t(\environment; \tilde{A}) +  \beta \E_t\left[(\overline{r}(A_\star) - \overline{r}(\tilde{A}))^2 \right] - \mathbb{I}_t(\tilde{A};(A_t, O_{t+1})) \\
=& \mathcal{L}_\beta(\tilde{A} | H_t) - \mathbb{I}_t(\tilde{A};(A_t, O_{t+1})).
\end{align*}
\end{dproof}

==> Blahut-Arimoto Satisficing Thompson Sampling/proofs/theorem2.tex <==
\begin{dproof}
From the inequalities satisfied by $\Gamma$, the Cauchy-Schwartz inequality, and Corollary \ref{co:cumulative-information}, we have
\begin{align*}
\E_\tau\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} (\overline{r}(\tilde{A}_t) - \overline{r}(A_t))\right]
\leq& \E_\tau\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} \sqrt{\Gamma \mathbb{I}_\tau(\tilde{A}_t; (A_t, O_{t+1}))} \right] \\
\leq& \sum_{t=\tau}^\infty \sqrt{\gamma^{2 (t-\tau)} \Gamma} \sqrt{\sum_{t=\tau}^\infty \E_\tau\left[\mathbb{I}_\tau(\tilde{A}_t; (A_t, O_{t+1}))\right]} \\
\leq& \sqrt{\Gamma \mc{L}_\beta(\tilde{A} | H_\tau) \sum_{t=0}^\infty \gamma^{2t}} \\
=& \sqrt{\frac{\Gamma \mc{L}_\beta(\tilde{A} | H_\tau)}{1-\gamma^2}}.
\end{align*}

Since $\mathcal{L}_\beta(\tilde{A}_t | H_t) \geq 0$,
$$\sqrt{\E_t\left[(\overline{r}(A_\star) - \overline{r}(\tilde{A}_t))^2 \right]} 
\leq (1-\gamma) \sqrt{\frac{\Gamma \mathcal{L}_\beta(\tilde{A}_t | H_t)}{1-\gamma^2}}.$$
Further, applying Jensen's inequality to the left-hand side and using the fact that $\tilde{A}_t$ minimizes $\mathcal{L}_\beta(\tilde{A}_t | H_t)$ on the right-hand side, 
$$\E_t\left[\overline{r}(A_\star) - \overline{r}(\tilde{A}_t) \right] 
\leq (1-\gamma) \sqrt{\frac{\Gamma \mathcal{L}_\beta(\tilde{A} | H_t)}{1-\gamma^2}}.$$
Lemma \ref{le:information-supermartingale} implies that
$$\E_\tau[\mathcal{L}_\beta(\tilde{A} | H_t)] \leq \mathcal{L}_\beta(\tilde{A} | H_\tau),$$
for all $t \geq \tau$, and therefore, by Jensen's inequality,
$$\E_\tau\left[\overline{r}(A_\star) - \overline{r}(\tilde{A}_t) \right]
\leq (1-\gamma) \E_\tau\left[\sqrt{\frac{\Gamma \mathcal{L}_\beta(\tilde{A} | H_t)}{1-\gamma^2}} \right] 
\leq (1-\gamma) \sqrt{\frac{\Gamma \E_\tau\left[\mathcal{L}_\beta(\tilde{A} | H_t) \right]}{1-\gamma^2}} 
\leq (1-\gamma) \sqrt{\frac{\Gamma \mathcal{L}_\beta(\tilde{A} | H_\tau)}{1-\gamma^2}}.$$
It follows that
\begin{align*}
\E_\tau\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} (\overline{r}(A_\star) - \overline{r}(\tilde{A}_t)) \right] \leq& \sqrt{\frac{\Gamma \mathcal{L}_\beta(\tilde{A} | H_\tau)}{1-\gamma^2}} \\
\leq& \sqrt{\frac{\Gamma (\mathbb{I}_\tau(\environment; \tilde{A}) + \beta \epsilon^2)}{1-\gamma^2}} \\
\leq& \sqrt{\frac{\Gamma \mathbb{I}_\tau(\environment; \tilde{A}) }{1-\gamma^2}} + \frac{\epsilon}{1-\gamma}.
\end{align*}

Applying these same steps, we complete the above bound as $$ \E_\tau\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} (\overline{r}(\tilde{A}_t) - \overline{r}(A_t))\right] \leq \sqrt{\frac{\Gamma \mathbb{I}_\tau(\environment; \tilde{A}) }{1-\gamma^2}} + \frac{\epsilon}{1-\gamma}.$$

Putting everything together, we have

\begin{align*}
    \E_\tau\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} (\overline{r}(A_\star) - \overline{r}(A_t))\right] &= \E_\tau\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} (\overline{r}(A_\star) - \overline{r}(\tilde{A}_t) + \overline{r}(\tilde{A}_t) - \overline{r}(A_t))\right] \\
    &= \E_\tau\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} (\overline{r}(A_\star) - \overline{r}(\tilde{A}_t))\right] + \E_\tau\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} (\overline{r}(\tilde{A}_t) - \overline{r}(A_t))\right] \\
    &\leq 2\sqrt{\frac{\Gamma \mathbb{I}_\tau(\environment; \tilde{A}) }{1-\gamma^2}} + \frac{2\epsilon}{1-\gamma}.
\end{align*}


% \begin{align*}
%     \E_\tau\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} (\overline{r}(A_\star) - \overline{r}(A_t))\right] &= \E_\tau\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} (\overline{r}(A_\star) - \overline{r}(\tilde{A}_t) + \overline{r}(\tilde{A}_t) - \overline{r}(A_t))\right] \\
%     &= \E_\tau\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} (\overline{r}(A_\star) - \overline{r}(\tilde{A}_t))\right] + \E_\tau\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} (\overline{r}(\tilde{A}_t) - \overline{r}(A_t))\right] \\
%     &\leq \E_\tau\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} (\overline{r}(A_\star) - \overline{r}(\tilde{A}_t))\right] + \E_\tau\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} \sqrt{\Gamma \mathbb{I}_\tau(\tilde{A}_t; (A_t, O_{t+1}))} \right] \\
%     &\leq \E_\tau\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} (\overline{r}(A_\star) - \overline{r}(\tilde{A}_t))\right] +  \sum_{t=\tau}^\infty \sqrt{\gamma^{2 (t-\tau)} \Gamma} \sqrt{\E_\tau\left[\sum_{t=\tau}^\infty \mathbb{I}_\tau(\tilde{A}_t; (A_t, O_{t+1}))\right]} \\
%     &\leq \E_\tau\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} (\overline{r}(A_\star) - \overline{r}(\tilde{A}_t))\right] + \sqrt{\Gamma \mc{L}_\beta(\tilde{A}_\tau|H_\tau) \sum_{t=0}^\infty \gamma^{2t}} \\
%     &\leq \E_\tau\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} (\overline{r}(A_\star) - \overline{r}(\tilde{A}_t))\right] + \sqrt{\frac{\Gamma \mathcal{L}_\beta(\tilde{A}_\tau | H_\tau)}{1-\gamma^2}} \\
%     &= \E_\tau\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} (\overline{r}(A_\star) - \overline{r}(\tilde{A}_t))\right] + \sqrt{\frac{\Gamma \left(\bI_\tau(\environment;\tilde{A}_\tau) + \beta\bE_\tau\left[(\overline{r}(A_\star) - \overline{r}(\tilde{A}_\tau))^2\right]\right)}{1-\gamma^2}} \\
%     &= \E_\tau\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} (\overline{r}(A_\star) - \overline{r}(\tilde{A}_t))\right] + \sqrt{\frac{\Gamma \mathbb{I}_\tau(\environment; \tilde{A}) }{1-\gamma^2}} + \sqrt{\frac{\Gamma \beta\bE_\tau\left[(\overline{r}(A_\star) - \overline{r}(\tilde{A}_\tau))^2\right]}{1-\gamma^2}} \\
%     &= \E_\tau\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} (\overline{r}(A_\star) - \overline{r}(\tilde{A}_t))\right] + \sqrt{\frac{\Gamma \mathbb{I}_\tau(\environment; \tilde{A}) }{1-\gamma^2}} + \frac{\sqrt{\bE_\tau\left[(\overline{r}(A_\star) - \overline{r}(\tilde{A}_\tau))^2\right]}}{1-\gamma} \\
%     &\leq \sqrt{\frac{\Gamma (\mathbb{I}(\environment; \tilde{A} |H_\tau = H_\tau) + \beta \epsilon^2)}{1-\gamma^2}} \\
%     &\leq \sqrt{\frac{\Gamma \mathbb{I}(\environment; \tilde{A} |H_\tau=H_\tau) }{1-\gamma^2}} + \frac{\epsilon}{1-\gamma}.
% \end{align*}
\end{dproof}


% \begin{proof}
% From the inequalities satisfied by $\Gamma$, the Cauchy-Schwartz inequality, and Corollary \ref{co:cumulative-information}, we have
% \begin{align*}
% \E\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} (\overline{r}(\tilde{A}_t) - \overline{r}(A_t)) \Big| H_\tau\right]
% \leq& \E\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} \sqrt{\Gamma \mathbb{I}(\tilde{A}_t; (A_t, O_{t+1}) | H_\tau=H_\tau)} \right] \\
% \leq& \sum_{t=\tau}^\infty \sqrt{\gamma^{2 (t-\tau)} \Gamma} \sqrt{\sum_{t=\tau}^\infty \E[\mathbb{I}(\tilde{A}_t; (A_t, O_{t+1}) | H_t = H_t) | H_\tau]} \\
% \leq& \sqrt{\Gamma \mathbb{I}(\environment; A_\star | H_\tau = H_\tau) \sum_{t=0}^\infty \gamma^{2t}} \\
% =& \sqrt{\frac{\Gamma \mathbb{I}(\environment; A_\star | H_\tau = H_\tau)}{1-\gamma^2}}.
% \end{align*}

% \dnote{Note that the above uses the Corollary 1 upper bound. Applying Corollary 2 instead, the bound is identical to the one below.}

% Since $\mathcal{L}_\beta(\tilde{A}_t | H_t) \geq 0$,
% $$\sqrt{\E\left[(\overline{r}(A_\star) - \overline{r}(\tilde{A}_t))^2 | H_t \right]} 
% \leq (1-\gamma) \sqrt{\frac{\Gamma \mathcal{L}_\beta(\tilde{A}_t | H_t)}{1-\gamma^2}}.$$
% Further, by Jensen's inequality and the fact that $\tilde{A}_t$ minimizes $\mathcal{L}_\beta(\tilde{A}_t | H_t)$, 
% $$\E\left[\overline{r}(A_\star) - \overline{r}(\tilde{A}_t) | H_t \right] 
% \leq (1-\gamma) \sqrt{\frac{\Gamma \mathcal{L}_\beta(\tilde{A} | H_t)}{1-\gamma^2}}.$$
% Lemma \ref{le:information-supermartingale} implies that
% $$\E[\mathcal{L}_\beta(\tilde{A} | H_t) | H_\tau] \leq \mathcal{L}_\beta(\tilde{A} | H_\tau),$$
% for all $t \geq \tau$, and therefore, by Jensen's inequality,
% $$\E\left[\overline{r}(A_\star) - \overline{r}(\tilde{A}_t) | H_\tau \right]
% \leq (1-\gamma) \E\left[\sqrt{\frac{\Gamma \mathcal{L}_\beta(\tilde{A} | H_t)}{1-\gamma^2}} \Big| H_\tau \right] 
% \leq (1-\gamma) \sqrt{\frac{\Gamma \E\left[\mathcal{L}_\beta(\tilde{A} | H_t) | H_\tau \right]}{1-\gamma^2}} 
% = (1-\gamma) \sqrt{\frac{\Gamma \mathcal{L}_\beta(\tilde{A} | H_\tau)}{1-\gamma^2}}.$$
% It follows that
% \begin{align*}
% \E\left[\sum_{t=\tau}^\infty \gamma^{t-\tau} (\overline{r}(A_\star) - \overline{r}(\tilde{A}_t)) \Big| H_\tau \right] \leq& \sqrt{\frac{\Gamma \mathcal{L}_\beta(\tilde{A} | H_\tau)}{1-\gamma^2}} \\
% \leq& \sqrt{\frac{\Gamma (\mathbb{I}(\environment; \tilde{A} |H_\tau = H_\tau) + \beta \epsilon^2)}{1-\gamma^2}} \\
% \leq& \sqrt{\frac{\Gamma \mathbb{I}(\environment; \tilde{A} |H_\tau=H_\tau) }{1-\gamma^2}} + \frac{\epsilon}{1-\gamma}.
% \end{align*}
% \end{proof}

==> Blahut-Arimoto Satisficing Thompson Sampling/proofs/theorem3.tex <==
\begin{dproof}
From the inequalities satisfied by $\Gamma$, the Cauchy-Schwartz inequality, and Corollary \ref{co:cumulative-information_undisc}, we have
\begin{align*}
\E_\tau\left[\sum_{t=\tau}^{T + \tau} \overline{r}(\tilde{A}_t) - \overline{r}(A_t)\right]
\leq& \sqrt{\Gamma} \E_\tau\left[\sum_{t=\tau}^{T + \tau} \sqrt{\mathbb{I}_\tau(\tilde{A}_t; (A_t, O_{t+1}))} \right] \\
\leq& \sqrt{\Gamma T \sum_{t=\tau}^{T + \tau} \E_\tau\left[\mathbb{I}_\tau(\tilde{A}_t; (A_t, O_{t+1}))\right]} \\
\leq& \sqrt{\Gamma T \mc{L}_\beta(\tilde{A} | H_\tau)}
\end{align*}

Since $\mathcal{L}_\beta(\tilde{A}_t | H_t) \geq 0$,
$$\sqrt{\E_t\left[(\overline{r}(A_\star) - \overline{r}(\tilde{A}_t))^2 \right]} 
\leq T^{-1} \sqrt{\Gamma T \mathcal{L}_\beta(\tilde{A}_t | H_t)}.$$
Further, applying Jensen's inequality to the left-hand side and using the fact that $\tilde{A}_t$ minimizes $\mathcal{L}_\beta(\tilde{A}_t | H_t)$ on the right-hand side, 
$$\E_t\left[\overline{r}(A_\star) - \overline{r}(\tilde{A}_t) \right] 
\leq T^{-1} \sqrt{\Gamma T \mathcal{L}_\beta(\tilde{A} | H_t)}.$$
Lemma \ref{le:information-supermartingale} implies that
$$\E_\tau[\mathcal{L}_\beta(\tilde{A} | H_t)] \leq \mathcal{L}_\beta(\tilde{A} | H_\tau),$$
for all $t \geq \tau$, and therefore, by Jensen's inequality,
$$\E_\tau\left[\overline{r}(A_\star) - \overline{r}(\tilde{A}_t) \right]
\leq T^{-1} \E_\tau\left[\sqrt{\Gamma T \mathcal{L}_\beta(\tilde{A} | H_t)} \right] 
\leq T^{-1} \sqrt{\Gamma T \E_\tau\left[\mathcal{L}_\beta(\tilde{A} | H_t) \right]} 
\leq T^{-1} \sqrt{\Gamma T \mathcal{L}_\beta(\tilde{A} | H_\tau)}.$$
It follows that
\begin{align*}
\E_\tau\left[\sum_{t=\tau}^{T + \tau} \overline{r}(A_\star) - \overline{r}(\tilde{A}_t) \right] \leq& \sqrt{\Gamma T \mathcal{L}_\beta(\tilde{A} | H_\tau)} \\
\leq& \sqrt{\Gamma T (\mathbb{I}_\tau(\environment; \tilde{A}) + \beta \epsilon^2)} \\
\leq& \sqrt{\Gamma T \mathbb{I}_\tau(\environment; \tilde{A})} + T\epsilon.
\end{align*}

Applying these same steps, we complete the above bound as $$ \E_\tau\left[\sum_{t=\tau}^{T + \tau} \overline{r}(\tilde{A}_t) - \overline{r}(A_t)\right] \leq \sqrt{\Gamma T \mathbb{I}_\tau(\environment; \tilde{A})} + T\epsilon.$$

Putting everything together, we have

\begin{align*}
    \E_\tau\left[\sum_{t=\tau}^{T + \tau} \overline{r}(A_\star) - \overline{r}(A_t)\right] &= \E_\tau\left[\sum_{t=\tau}^{T + \tau} \overline{r}(A_\star) - \overline{r}(\tilde{A}_t) + \overline{r}(\tilde{A}_t) - \overline{r}(A_t)\right] \\
    &= \E_\tau\left[\sum_{t=\tau}^{T + \tau} \overline{r}(A_\star) - \overline{r}(\tilde{A}_t)\right] + \E_\tau\left[\sum_{t=\tau}^{T + \tau} \overline{r}(\tilde{A}_t) - \overline{r}(A_t)\right] \\
    &\leq 2\sqrt{\Gamma T \mathbb{I}_\tau(\environment; \tilde{A})} + 2T\epsilon.
\end{align*}
\end{dproof}

